Sharp bounds for joint moments of the Riemann zeta function

In previous work, the first author obtained conjecturally sharp upper bounds for the joint moments of the $(2k-2h)^{\text{th}}$ power of the Riemann zeta function with the $2h^{\text{th}}$ power of its derivative on the critical line in the range $1\leq k \leq 2$, $0 \leq h \leq 1$. Unconditionally, we extend these upper bounds to all $0 \leq h\leq k \leq 2$, and obtain lower bounds for all $0\leq h \leq k+1/2$. Assuming the Riemann hypothesis, we give sharp bounds for all $0\leq h \leq k$. We also prove upper bounds of the conjectured order for more general joint moments of zeta with its higher derivatives.

==> introduction2.tex <==
\section{Introduction}
This paper is concerned with the joint moments of the Riemann zeta function with its derivative on the critical line and other natural variants of these moments.
Work of Keating and Snaith \cite{KS2, KS1}, Hughes \cite{Hughes}, and Hall \cite{hall} has led to the conjecture that for $k > -\tfrac{1}{2}$ and $-\tfrac{1}{2} < h \leq k + \tfrac{1}{2}$,
\begin{equation} \label{eqn:JMConjecture}
\int_{T}^{2T} |\zeta(\tfrac{1}{2} + i t)|^{2k - 2 h} \left|\zeta'(\tfrac{1}{2} + i t)\right|^{2h} \ dt \sim C(k,h) T (\log T)^{k^2 + 2h} 
\end{equation}
as $T \rightarrow \infty$ for certain constants $C(k,h)$.
These constants can be expressed as the product of a natural number theoretic factor and a factor coming from conjectural connections of the Riemann zeta function with random matrix theory.
The arithmetic factor is given by a product over primes, while the random matrix factor can be expressed using Painlevé trancendents.
For finite $N$, the random matrix factor can be expressed using the solution to a Painlevé V differential equation \cite{P5}, while the random matrix factor in the limit $N\rightarrow \infty$ is related to the solution of a Painlevé III differential equation \cite{AKW, BBBCPRS, P5, FW}.
This asymptotic (\ref{eqn:JMConjecture}) is currently only known to hold for integer $h , k$ satisfying $0 \leq h \leq k \leq 2$ due to work of Ingham \cite{Ingham} and Conrey \cite{Conrey}.

Since the asymptotic (\ref{eqn:JMConjecture}) seems out of reach for all remaining values of $h$ and $k$, it is natural to ask if we can at least obtain upper bounds of the right order.
The work of Heap, Radziwiłł, and Soundararajan \cite{heap-radziwill-soundararajan} shows that we have upper bounds of the expected order for (\ref{eqn:JMConjecture}) for $h = 0, k \leq 2$. 
In fact, lower bounds of the conjectured order are also known for all $k \geq 0$ when $h = 0$ due to work of Heap and Soundararajan \cite{heap-soundararajan}. 
By using Conrey's asymptotic for the fourth moment of the derivative of zeta \cite{Conrey} along with Hölder's inequality, one also sees that an upper bound of the expected order for (\ref{eqn:JMConjecture}) holds for $k = 2$ and $h \leq 2$.
Finally, the first author recently showed \cite{curran-1} that the an upper bound of the expected order for (\ref{eqn:JMConjecture}) holds in the larger range where $0\leq h\leq 1$ and $1\leq k \leq 2$.
The paper \cite{curran-1} uses the work of Heap, Radziwiłł, and Soundararajan \cite{arguin-ouimet-radziwill} along with the observation that if we have an upper bound of the expected order in (\ref{eqn:JMConjecture}) for a given pair $k, h$, then we also have an upper bound of the expected order for the pair $k, h'$ for any $0\leq h' \leq h$.
This latter observation is a simple consequence of Hölder's inequality and will be quite useful in this paper.

Our primary aim is to prove the upper bound (\ref{eqn:JMConjecture}) for all $0 \leq h \leq k \leq 2$. 
The method of proof extends to the higher derivatives.

\begin{theorem} \label{thm:mainUnconditional}
Let $0\leq h \leq k \leq 2$. Then
\[
\int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \ll T (\log T)^{k^2 + 2 h}.
\]
\end{theorem}

% \begin{rmk}
% The method here can be generalized in a straightforward manner to provide sharp bounds for the joint moments of the  $(2k-2h)^{\text{th}}$ power of $\zeta$ with the $2h^{\text{th}}$ power of $\zeta^{(n)}$ for all natural numbers $n$, but we focus on the case of $n = 1$ for simplicity.
% \end{rmk}
\noindent 
In fact our proof easily generalizes to give upper bounds for joint moments of zeta with its higher order derivatives.
Assuming the Riemann hypothesis, the bound extends to all $0 \leq h \leq k$.

\begin{theorem}\label{thm:mainRH}
Suppose that $k \geq 1/2$, $h_j \geq 0$ for $1\leq j \leq m$, and $h_1 + \cdots + h_m \leq k$. Then
\begin{equation*}\label{eq:generalMM}
        \int_{T}^{2T}|\zeta(\half+it)|^{2k-2\sum_{j=1}^m h_j}\prod_{j=1}^m|\zeta^{(j)}(\half+it)|^{2h_j} \ dt\ll_{k, h_j} T(\log T)^{k^2 + 2\sum_{j=1}^m j h_j},
    \end{equation*}
    where  we assume the Riemann hypothesis when $k > 2$.
\end{theorem}

\noindent
The upper bound in Theorem \ref{thm:mainRH} is the same order of magnitude one would predict using random matrix theory. The case of integral joint moments of a product of two derivatives of characteristic random unitary matrices has been extensively studied by Keating and Wei \cite{keating-wei-1,keating-wei-2}.

Combining Theorems \ref{thm:mainUnconditional} and  \ref{thm:mainRH},
we have upper bounds of the expected order in (\ref{eqn:JMConjecture}) for all $0 \leq h \leq k$ assuming the Riemann hypothesis.
We also obtain lower bounds for all $k \geq 0$ and $0\leq h \leq k + \tfrac{1}{2}$, so the upper bounds for (\ref{eqn:JMConjecture}) are of the correct order.
\begin{theorem} \label{thm:lowerJM}
If $k \geq 0$ and $0\leq h \leq k + \tfrac{1}{2}$ then
\[
\int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \gg_{k,h} T (\log T)^{k^2 + 2 h}.
\]
\end{theorem}

\noindent
We will begin by showing that Theorem \ref{thm:lowerJM} is a short consequence of the lower bounds for the $2k^\text{th}$ moments of zeta for $k \geq 0$ obtained by Heap and Soundararajan \cite{heap-soundararajan}.
The argument we give is essentially the same argument used in Conrey's \cite{Conrey} proof of the explicit lower bound
\[
\int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^{3} |\zeta'(\tfrac{1}{2} + i t)| \ d t \geq (1 + o(1)) \frac{173}{672\pi^2} T (\log T)^5.
\]
Since obtaining good implicit constants is not our concern in this paper, a slightly simpler version of the argument in \cite{Conrey} will suffice.

We will then move onto proving the upper bounds.
The proof of Theorem \ref{thm:mainUnconditional} splits into two cases.
Using Hölder's inequality, it suffices to prove Theorem \ref{thm:mainUnconditional} first in the case where $1\leq h \leq k \leq 2$, and then in the case where $0 \leq h \leq k \leq 1$.
When $1\leq h \leq k \leq 2$, we will represent the derivative of zeta by a contour integral and can use Hölder's or Jensen's inequality to essentially bound (\ref{eqn:JMConjecture}) by $(\log T)^{2h}$ times the $2k^\text{th}$ moment of zeta.
The argument here is similar to one in work of Milinovich \cite{Mili} on moments of derivatives of zeta, and the proof fails for small $h$ because $x \mapsto x^{2h}$ is not convex when $h < 1/2$.
We will use this same technique to prove Theorem \ref{thm:mainRH}.

To prove Theorem \ref{thm:mainUnconditional} when $0 \leq h \leq k \leq 1$, we will use the work of Heap, Radziwiłł, and Soundararajan \cite{heap-radziwill-soundararajan} to bound the $(2k-2h)^\text{th}$ power of zeta by the square of zeta times the exponential of a Dirichlet polynomial plus the exponential of another Dirichlet polynomial.
A key difference between our method and the one in \cite{heap-radziwill-soundararajan} is that we will first decompose the interval $[T,2T]$, and then apply a separate interpolation inequality on each piece of the decomposition.
This trick allows us to circumvent the issue of bounding non-integer moments of Dirichlet polynomials. 
Finally we will bound the exponentials of Dirichlet polynomials using the method in \cite{heap-radziwill-soundararajan} to reduce our theorem to a variety of twisted moment calculations, all of which are essentially computed in either \cite{curran-1} or \cite{heap-radziwill-soundararajan}.


 
\section*{Acknowledgements}
\noindent
Part of this work was written during a visit by the first author to the University of Manchester. He would like to thank Hung Bui and that institution for their hospitality and support, as well as his advisor Jon Keating for useful comments. The second author would like to thank his advisor Hung Bui for helpful discussions. Finally both authors would like to thank Winston Heap for comments on an early draft of the paper, and to thank Soundararajan for bringing the argument in \cite{Conrey} to their attention.

==> lower_bounds.tex <==
\section{Lower Bounds: Proof of Theorem \ref{thm:lowerJM}}

We begin by writing
\[
\int_T^{2T}|\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t =\int_T^{2T}|\zeta(\tfrac{1}{2} + i t)|^{2k} \left(\left|\Re \frac{\zeta'}{\zeta}(\tfrac{1}{2}+ i t)\right|^2+ \left|\Im \frac{\zeta'}{\zeta}(\tfrac{1}{2}+ i t)\right|^2\right)^{h} \ d t
\]
It is a standard consequence of Stirling's approximation and the functional equation that
\[
\Re \frac{\zeta'}{\zeta}(\tfrac{1}{2}+ i t) = -\frac{1}{2}\log\frac{t}{2\pi} + O(|t|^{-1}).
\]
Therefore for large $T$
\[
\int_T^{2T}|\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \gg (\log T)^{2h} \int_T^{2T}|\zeta(\tfrac{1}{2} + i t)|^{2k}  \ d t.
\]
Theorem \ref{thm:lowerJM} now follows after an application of the main theorem in \cite{heap-soundararajan}. \qed

==> notation.tex <==
\subsection{Proof of Theorem \ref{thm:mainUnconditional}: $h \leq k \leq 1$ case} 

We will first set up our notation.
Throughout our parameters will depend on the value of $k$.
Denote, $k_\ast = \max(k,1)$,
Let $\log_j$ denote the $j$-fold iterated logarithm, set $T_0 = 1$,
\[
T_j := \exp\left(\frac{\log T}{k_\ast^2(\log_{j+1} T)^2}\right)
\]
for $j \geq 1$, and 
\[
J := \max\left\{j : \log_j T \geq 10^4 \right\}.
\]
For $1\leq j \leq J$ set
\[
\p_j(s) := \sum_{T_{j-1} < p \leq T_{j} } \frac{1}{p^s}, \quad P_j := \sum_{T_{j-1} < p \leq T_{j} } \frac{1}{p}.
\]
Next define the Dirichlet polynomials
\[
\n_j(s;\b) = \sum_{\substack{p \mid n \Rightarrow p\in (T_{j-1},T_j] \\ \Omega(n) \leq 10 k_\ast^2 K_j}} \frac{\b^{\Omega(n)} g(n)}{n^s},
\]
where $|\b| \leq k_\ast$,
\[
K_j := 50 P_j, \  g(n) = \prod_{p^r \| n}\tfrac{1}{r!},\ \text{ and } \Omega(n) = \sum_{p^r \| n} r.
\]
Note $\n_j(s;\b)$ is a Dirichlet polynomial of length $\leq T_j^{500k_\ast^2 P_j}$, so $\prod_{j \leq J}\n_j(s;\b)$ has length at most $T_1^{500k_\ast^2 P_1} T_2^{500k_\ast^2 P_2} \cdots T_J^{500 k_\ast^2 P_J} \leq T^{1/10}$. 


We will decompose the interval $[T,2T]$ depending on the sizes of the $\p_j(s)$. Define the good set
\[
\G := \left\{t\in [T,2T] : |\p_j(\tfrac{1}{2} + i t)| \leq K_j \text{ for all } j \leq J \right\},
\]
and the bad sets
\[
\B_r := \{t\in [T,2T]: |\p_j (\tfrac{1}{2}+ i t)| \leq K_j \text{ for all } 1\leq j < r \text{ but } |\p_{r} (\tfrac{1}{2} + i t)|  > K_{r} \}.
\]
A similar decomposition occurs in the work of Harper \cite{harper} and also occurs implicitly in the work of Radziwiłł and Soundararajan \cite{radziwill-soundararajan} and related papers \cite{curran-1, heap-radziwill-soundararajan, heap-soundararajan}.
In our argument, it will be important to keep careful track of which values $t$ are good or bad because we will use a separate interpolation inequality on each set of our partition of $[T,2T]$. This will allow us to avoid having to calculate non-integer moments of Dirichlet polynomials.
While we could compute non-integer moments in the same manner as Heap and Soundararajan  do in \cite{heap-soundararajan}, circumventing these calculations will simplify our proof.
Throughout we will use the following lemmata, which are essentially contained in Proposition 1 of \cite{heap-radziwill-soundararajan}.

\begin{lemma}\label{lem:interpol}
For $0\leq \b \leq 1$ and $r \leq J +1$,
\[
|\zeta(s)|^{2\b} \ll |\zeta(s)|^2 \exp\left((2\b-2) \sum_{j < r} \Re \p_j(s)\right) + \exp\left(2\b \sum_{j < r} \Re \p_j(s)\right).
\]
\end{lemma}
\begin{proof}
This is an immediate consequence of Young's inequality $xy \leq x^p / p + y^q / q$ for $x,y\geq 0$ and conjugate exponents $p,q > 1$, noting that the result is trivial when $\b$ is 0 or 1.
\end{proof}

\begin{lemma}\label{lem:taylorExp}
If $|\b| \leq k_\ast$, $j \leq J$ and $|\p_j(s) | \leq K_j$, then
\[
\exp\left(2\b \Re \p_j(s)\right) = (1 + O(e^{- k_\ast^2 P_j})) |\n_j(s; \b)|^2.
\]
\end{lemma}
\begin{proof}
By Taylor expansion the exponential up to the $10 k_\ast^2 K_j^\text{th}$ term we find
\[
\left|\exp(\b \p_j(s)) - \n_j(s;\b)\right| \leq e^{-10 k_\ast^2  K_j}
\]
since $|\b \p_j(s)| \leq  k_\ast K_j$.
Therefore
\[
\exp\left(2\b \Re \p_j(s)\right) = |\exp(\b \p_j(s)|^2 = |\n_j(s;\b) + \theta e^{-20 k_\ast^2 K_j}|^2
\]
where $\t$ denotes a quantity depending on $s$ with $|\t|\leq 1$.
Finally by assumption $|\exp(\b \p_j(s))| \geq e^{-k_\ast^2 K_j}$ and therefore also $|\n_j(s;\b)| \geq e^{-k_\ast^2 K_j/2}$, so we may turn the additive error into a multiplicative error.
\end{proof}

==> old/proof_RH.tex <==
\subsection{Proof of Theorem \ref{thm:mainRH}}

This brief section will be very similar to the proof of Theorem \ref{thm:mainUnconditional} in the range $h \geq 1$.
% The argument here earlier was confusing to me, so I've simplified it a bit.
First note that we may assume that each $h_j \geq 1/2$.
Indeed if we assume that (\ref{eq:generalMM}) holds for $h_j \geq 1/2$ and $k \geq h_1 + \cdots + h_m$, then because the exponents on the right hand side of (\ref{eq:generalMM}) are linear in the $h_j$ Hölder's inequality implies that (\ref{eq:generalMM}) also holds in the larger range where $h_j \geq 0$, $k \geq m/2$, and $k \geq h_1 + \cdots + h_m$.

Starting from
\begin{equation*}
    \zeta^{(n)}(s)=\frac{n!}{2\pi i }\int_{|z|= 1/\log T} \frac{\zeta(s+z)}{z^{n+1}} \ d z,
\end{equation*}
% Changed j to n
we instead find that
\begin{align*}
    \int_{T}^{2T} &|\zeta(\tfrac{1}{2}+it)|^{2k-2\sum_{j=1}^m h_j}\prod_{j=1}^m|\zeta^{(n_j)}(\tfrac{1}{2}+it)|^{2h_j}\ d t \\
    &\ll \int_T^{2T}|\zeta(\tfrac{1}{2}+it)|^{2k-2\sum_{j=1}^m h_j} \left|\prod_{j=1}^m \int_{|z_j|= 1/\log T} \frac{|\zeta(\half+it+z_j)|}{|z_j|^{n_j+1}} \ d |z_j|\right|^{2h_j}\ d t.
\end{align*}

Since each $h_j \geq 1/2$, Jensen's inequality bounds this by
\begin{align*}
    &\ll (\log T)^{2\sum_{j=1}^m n_j h_j}\max_{|z_j|= 1/\log T}\int_T^{2T} |\zeta(\half+it)|^{2k-2\sum_{j=1}^m h_j} \prod_{j=1}^m|\zeta(\half+it+z_j)|^{2h_j}\ d t.
\end{align*}
Now using H\"older's inequality to separate out the shifts, this is at most
\begin{equation*}
    \ll (\log T)^{2\sum_{j=1}^m n_j h_j} \max_{|z_j|= 1/\log T} \left(\int_{T}^{2T}|\zeta(\half+it)|^{2k}\right)^{1-\sum_{j=1}^m h_j/k}\prod_{j=1}^m\left(\int_{T}^{2T}|\zeta(\half+it+z_j)|^{2k}\ d t \right)^{h_j/k}.
\end{equation*}
%Fixed the exponent on the first integral
By the same argument we used to prove Theorem \ref{thm:mainUnconditional} (using Harper's conditional bound on the moments of zeta \cite{harper} instead of the unconditional estimate of Heap, Radziwiłł, and Soundararajan \cite{heap-radziwill-soundararajan}), each of the above shifted $2k^\text{th}$ moments is $\ll T(\log T)^{k^2}$ uniformly in $|z_j| = 1/\log T$, so Theorem \ref{thm:mainRH} follows. \qed 


% This brief section will be very similar to the proof of Theorem \ref{thm:mainUnconditional} in the range $h \geq 1$.
% % The argument here earlier was confusing to me, so I've simplified it a bit.
% First note that we may assume that each $h_j \geq 1/2$.
% Indeed if we assume that (\ref{eq:generalMM}) holds for $h_j \geq 1/2$ and $k \geq h_1 + \cdots + h_m$, then because the exponents on the right hand side of (\ref{eq:generalMM}) are linear in the $h_j$ Hölder's inequality implies that (\ref{eq:generalMM}) also holds in the larger range where $h_j \geq 0$, $k \geq m/2$, and $k \geq h_1 + \cdots + h_m$.
% %In the event that for some $1\leq r \leq m$ we have $h_r\leq 1/2$, by H\"older's inequality it is instead sufficient to estimate the same moment but with $h_r$ replaced by some $k-\sum_{j\neq r}h_j>\alpha_r>1/2$:
% %\begin{equation*}
%     %\begin{split}
%     %\int_{T}^{2T} |\zeta (\half+ & it)|^{2k - 2\sum_{j=1}^m h_j} \prod_{j=1}^m |\zeta^{(j)}(\half+it)|^{2h_j} \ d t\\
%     %\ll &\left(\int_{T}^{2T}|\zeta(1/2+it)|^{2k-2\alpha_r-2\sum_{j\neq r}h_j} |\zeta^{(r)}(\half+it)|^{2\alpha_r}\prod_{j\neq r} |\zeta^{(j)}(\half+it)|^{2h_j}\right)^{h_r/\alpha_r}\\
%     %& \times\left(\int_{T}^{2T}|\zeta(1/2+it)|^{2k-2\alpha_r-2\sum_{j\neq r}h_j}\prod_{j\neq r} |\zeta^{(j)}(\half+it)|^{2h_j}\right)^{1-h_r/\alpha_r}.
%     %\end{split}
% %\end{equation*}
% %We iterate this process as necessary over $1\leq j \leq m$. The conditions on $k$ ensure that we can choose each $\alpha_j>1/2$ and such that $\sum_{\alpha_j} < k$. It thus suffices to obtain the upper bound in Theorem \ref{thm:mainRH} for the moments where each $h_j$ is either zero or $h_j\geq 1/2$.
% Starting from
% \begin{equation*}
%     \zeta^{(j)}(s)=\frac{j!}{2\pi i }\int_{|z|= 1/\log T} \frac{\zeta(s+z)}{z^{j+1}} \ d z,
% \end{equation*}
% % Changed j to j + 1
% we instead find that
% \begin{align*}
%     \int_{T}^{2T} &|\zeta(\tfrac{1}{2}+it)|^{2k-2\sum_{j=1}^m h_j}\prod_{j=1}^m|\zeta^{(j)}(\tfrac{1}{2}+it)|^{2h_j}\ d t \\
%     &\ll \int_T^{2T}|\zeta(\tfrac{1}{2}+it)|^{2k-2\sum_{j=1}^m h_j} \left|\prod_{j=1}^m \int_{|z|_j= 1/\log T} \frac{|\zeta(\half+it+z_j)|}{|z_j|^{j+1}} \ d |z_j|\right|^{2h_j}\ d t.
% \end{align*}
% % Made slight corrections because z^{j+1} is in the denominator instead of  z^j. (this is because dz/z is the measure that's scaling invariant)
% % I switched  the -2 in the exponent of log T to a plus 2
% % It's standard practice to just type $\ d$ instead of using the \dd command you made.
% Since each $h_j \geq 1/2$, Jensen's inequality bounds this by
% \begin{align*}
%     &\ll (\log T)^{2\sum_{j=1}^m jh_j}\max_{|z_j|= 1/\log T}\int_T^{2T} |\zeta(\half+it)|^{2(k-h_1 - \cdots - h_m)} \prod_{j=1}^m|\zeta(\half+it+z_j)|^{2h_j}\ d t.
% \end{align*}
% Now using H\"older's inequality to separate out the shifts, this is at most
% \begin{equation*}
%     \ll (\log T)^{2\sum_{j=1}^m jh_j} \max_{|z_j|= 1/\log T} \left(\int_{T}^{2T}|\zeta(\half+it)|^{2k}\right)^{1-\sum_{j=1}^m h_j/k}\prod_{j=1}^m\left(\int_{T}^{2T}|\zeta(\half+it+z_j)|^{2k}\ d t \right)^{h_j/k}.
% \end{equation*}
% %Fixed the exponent on the first integral
% By the same argument we used to prove Theorem \ref{thm:mainUnconditional} (using Harper's conditional bound on the moments of zeta \cite{harper} instead of the unconditional estimate of Heap, Radziwiłł, and Soundararajan \cite{heap-radziwill-soundararajan}), each of the above shifted $2k^\text{th}$ moments is $\ll T(\log T)^{k^2}$ uniformly in $|z_j| = 1/\log T$, so Theorem \ref{thm:mainRH} follows. \qed 

==> proof_RH_new.tex <==
%Made some small edits here to remove the n_j's from the notation

\section{Conditional upper bounds}
We will now prove Theorem \ref{thm:mainRH}.
This is essentially the same as the proof of Theorem \ref{thm:mainUnconditional} when $h \geq 1/2$.
For simplicity we will write $h = h_1 + \cdots + h_m$.
First, apply H\"older's inequality to separate out each derivative:
    \begin{multline}\label{eq:RH_Thm_FirstHolder}
        \int_{T}^{2T}|\zeta(\half+it)|^{2k-2h}\prod_{j=1}^m|\zeta^{(j)}(\half+it)|^{2h_j} \ dt \\
         \ll \left(\int_{T}^{2T}|\zeta(\half+it)|^{2k}\ dt\right)^{1-h/k} \times \prod_{j=1}^m \left(\int_T^{2T} |\zeta^{(j)}(\half+it)|^{2k} \ dt \right)^{h_j/k}.
    \end{multline}
    The result then follows once we show that, for any fixed $j\in\Z_{>0}$
    \begin{equation}\label{eq:RH_Thm.1}
        \int_{T}^{2T} |\zeta^{(j)}(\half+it)|^{2k}\ dt\ll T(\log T)^{k^2+2jk}.
    \end{equation}
    For $t\in[T,2T]$ we have that
    \begin{equation*}
        \zeta^{(j)}(\half+it) = \frac{1}{2\pi i}\oint_{|z|=1/\log T} \frac{\zeta(\half+it+z)}{z^{j+1}}\ dz.
    \end{equation*}
    Applying this to the moment in \eqref{eq:RH_Thm.1} and arguing as in Section \ref{sec:big_h_proof} yields
    \begin{align*}
        \int_{T}^{2T} |\zeta^{(j)}(\half+it)|^{2k}\ dt 
        &\ll (\log T)^{2jk}\int_{T}^{2T} \left|\oint_{|z|=1/\log T}|\zeta(\half+it+z)| \ \frac{d |z|}{|z|} \right|^{2k} \ dt \\
        &\ll (\log T)^{2jk} \max_{|z|=1/\log T}\int_T^{2T} |\zeta(\half+it+z)|^{2k}\ dt,
    \end{align*}
    with the penultimate step by H\"older's inequality. Finally, the shifted moments is  $\ll T (\log T)^{k^2}$ uniformly in $z$. This again uses the corresponding argument in Section \ref{sec:big_h_proof}, appealing to Harper's bound \citep{harper} for the range $k>2$ instead of Theorem 1 in \citep{heap-radziwill-soundararajan}.
    Inserting these bounds into the right hand side of \eqref{eq:RH_Thm_FirstHolder} proves Theorem \ref{thm:mainRH}. 
    \qed

==> proof_big_k2.tex <==
\section{Unconditional Upper Bounds}

\subsection{Proof of Theorem \ref{thm:mainUnconditional}: $h \geq 1$ case}\label{sec:big_h_proof}

The starting point of the proof is the formula
\[
\zeta'(s) = \frac{1}{2\pi i} \int_{|z| = 1/\log T} \frac{\zeta(s+z)}{z^2} dz.
\]
A couple of applications of Hölder's inequality give
\begin{align*}
\int_T^{2T} |\zeta&(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t\\
&\ll \int_T^{2T} |\zeta(\half+it)|^{2k-2h} \left(\int_{|z|=1/\log T}\frac{|\zeta(\half+it+z)|}{|z|^2} \ d|z| \ dt \right)^{2h}\\
&\ll (\log T)^{2h} \max_{|z|= 1/\log T} \int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta(\tfrac{1}{2} + i t + z)|^{2h} \ d t\\
&\ll (\log T)^{2h} \max_{|z|= 1/\log T} \left(\int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^{2k} \ d t \right)^{1-h/k} \left(\int_T^{2T} |\zeta(\tfrac{1}{2} + i t + z)|^{2k} \ d t \right)^{h/k}.
\end{align*}
The first integral may be bounded by $\ll T(\log T)^{k^2}$ by Theorem 1 of \cite{heap-radziwill-soundararajan}. 
The second integral may also be bounded by $\ll T(\log T)^{k^2}$ uniformly in $|z| = 1/\log T$. 
To see this, we may reduce to the case that $\Re z \geq 0$ by using the functional equation (see Lemma 22 of \cite{FHKConjecture}).
The claim now follows from combining Theorem 1 of  \cite{heap-radziwill-soundararajan} and Theorem 7.1 of  \cite{Titchmarsh} with Theorem 2 of \cite{Gabriel}.
While Theorem 2 of Gabriel's paper \cite{Gabriel} only holds for functions analytic in a strip, we may still use his result by approximating the indicator function of the rectangle $1/2 \leq \sigma \leq 3/2, T \leq t \leq 2T$ by a suitable analytic function, see Lemma 3.5 of \cite{arguin-ouimet-radziwill}.
Alternatively, one may show this follows by a straightforward modification of the argument in \cite{heap-radziwill-soundararajan}.
This concludes the proof when $h \geq 1$, and in fact when $h \geq 1/2$. \qed

% This might be worth mentioning, as it also gets some of the small k range with minimal effort. (2023-05-01)
% I'm just going to mention this in the introduction because this is the idea I used in my joint moments paper.

%Furthermore, as long as $k>1/2$, this can also prove Theorem \ref{thm:mainUnconditional} for any $h\in(0,k)$. For any $\alpha$ satisfying $1/2,h<\alpha<k$, by H\"older's inequality we have
%\begin{equation}\label{eq:alpha-holder}
%    \begin{split}
%        \int_T^{2T}&|\zeta(1/2+it)|^{2k-2h}|\zeta'(1/2+it)|^{2h} \dd t\\ &\leq 
%        \left(\int_{T}^{2T}|\zeta(1/2+it)|^{2k-2\alpha}|\zeta'(1/2+it)|^{2\alpha}\dd t\right)^{h/\alpha}\left(\int_{T}^{2T}|\zeta(1/2+it)|^{2k}\dd t\right)^{1-h/\alpha}.
%    \end{split}
%\end{equation}
%Hence the upper bound in the $h\geq 1/2$ range along with theorem 1 in \citep{heap-radziwill-soundararajan} sharply bound the left hand side of \eqref{eq:alpha-holder}.
%%%


==> proof_small_k2.tex <==


The proof of Theorem \ref{thm:mainUnconditional} for $0 \leq h \leq k \leq 1$ will follow from the bounds 
\begin{equation*} \label{eq:GoodSetBound}
\int_\G |\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \ll T (\log T)^{k^2 + 2 h}
\end{equation*}
and
\begin{equation*} \label{eq:badSetBound}
\int_{\B_r} |\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \ll T (\log T)^{k^2 + 2 h}  e^{-10 P_r}
\end{equation*}
after summing over $1 \leq r \leq J$.
To bound joint moments over the good set, we will apply Lemma \ref{lem:interpol} with $r = J + 1$:
\begin{align*}
\int_\G |\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} &|\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \\
\ll &\int_\G |\zeta(\tfrac{1}{2} + i t)|^2 |\zeta'(\tfrac{1}{2} + i t)|^{2h} \exp\left(2(k-h-1) \sum_{j\leq J}\Re \p_j(\tfrac{1}{2} + i t)\right) \ d t \\
&+ \int_\G |\zeta'(\tfrac{1}{2} + i t)|^{2h}  \exp\left(2(k-h) \sum_{j\leq J} \Re \p_j(\tfrac{1}{2} + i t)\right) \ d t.
\end{align*}
Now applying Hölder's inequality, then Lemma \ref{lem:taylorExp}, and finally extending the range of integration to all of $[T,2T]$ for both summands we find
\begin{align} 
\int_\G |\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} &|\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \nonumber \\
\ll \Bigg( &\int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^2 |\zeta'(\tfrac{1}{2} + i t)|^{2} \prod_{j\leq J} |\n_j(\tfrac{1}{2} + i t;k-2)|^2 \ d t \Bigg)^h \label{eq:1}\\
&\qquad\times \Bigg( \int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^2 \prod_{j\leq J} |\n_j(\tfrac{1}{2}+ i t;k - 1)|^2 \ d t \Bigg)^{1-h} \label{eq:2}
\\
 + & \Bigg( \int_T^{2T} |\zeta'(\tfrac{1}{2} + i t)|^{2} \prod_{j\leq J} |\n_j(\tfrac{1}{2} + i t;k-1)|^2 \ d t \Bigg)^h \label{eq:3} \\
&\qquad\times \Bigg( \int_T^{2T}  \prod_{j\leq J} |\n_j(\tfrac{1}{2}+ i t;k )|^2 \ d t \Bigg)^{1-h} \label{eq:4}.
\end{align}
Here we have used that $\prod_{j\leq J}(1+O(e^{-P_j})) = O(1)$.
The order in which we apply Hölder's inequality and Lemma \ref{lem:taylorExp} is crucial here, for when the dust settles all of the Dirichlet polynomials are simply raised to the power two.

The moments over the sets $\B_r$ are handled in a completely analogous manner --- the only differences are that we apply Lemma \ref{lem:interpol} with the sum truncated at $r$ instead of $J+1$ and that we multiply the integrand by $|\p_r(s)/50 P_r|^{2\ceil{50P_r}}$ before extending the range of integration to all of $[T,2T]$.
The corresponding inequality obtained is 
\begin{align}
\int_{\B_r} |\zeta(\tfrac{1}{2} + i t)&|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \nonumber \\
\ll \Bigg( \int_T^{2T} &|\zeta(\tfrac{1}{2} + i t)|^2 |\zeta'(\tfrac{1}{2} + i t)|^{2} \prod_{j < r} |\n_j(\tfrac{1}{2} + i t;k-2)|^2 \left|\frac{\p_r(s)}{50 P_r} \right|^{2\ceil{50P_r}} \ d t \Bigg)^h \label{eq:5}\\
&\qquad \times \Bigg( \int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^2 \prod_{j < r} |\n_j(\tfrac{1}{2}+ i t;k - 1)|^2 \left|\frac{\p_r(s)}{50 P_r} \right|^{2\ceil{50P_r}} \ d t \Bigg)^{1-h} \label{eq:6}
\\
+ \Bigg( &\int_T^{2T} |\zeta'(\tfrac{1}{2} + i t)|^{2} \prod_{j < r} |\n_j(\tfrac{1}{2} + i t;k-1)|^2 \left|\frac{\p_r(s)}{50 P_r} \right|^{2\ceil{50P_r}} \ d t \Bigg)^h \label{eq:7} \\
&\qquad\times \Bigg( \int_T^{2T}  \prod_{j < r} |\n_j(\tfrac{1}{2}+ i t;k )|^2 \left|\frac{\p_r(s)}{50 P_r} \right|^{2\ceil{50P_r}} \ d t \Bigg)^{1-h}. \label{eq:8}
\end{align}
Thus the problem is reduced to a handful of twisted moment or mean value calculations.
Since all the Dirichlet polynomials appearing have length at most $T^{1/4-\ve}$ we may bound (\ref{eq:1}) and (\ref{eq:5}) with Proposition 2.5 of \cite{curran-1}, and we may bound (\ref{eq:3}) and (\ref{eq:7}) with Proposition 2.4 of \cite{curran-1} (while these propositions are only stated for $1\leq k \leq 2$, they are still valid in the range $0\leq k \leq 2$).
We may bound (\ref{eq:4}) and (\ref{eq:8}) with Proposition 2 of \cite{heap-radziwill-soundararajan},
and we may bound \eqref{eq:2} with Proposition 2 of \cite{heap-soundararajan}. The only moment left to evaluate is \eqref{eq:6}, which can be quickly computed using the formulae in \cite{curran-1}.
Before we proceed with the calculation, given a Dirichlet polynomial $A(s) = \sum_{h\leq T^\theta} a_h h^{-s}$ with $\theta < 1/2$, define
\[
F(z_1,z_2) = \sum_{h,k \leq T^\theta} \frac{a_h \overline{a_k}}{[h,k]} \frac{(h,k)^{z_1 + z_2}}{h^{z_1} k^{z_2}}.
\]
%which is still a second moment of the zeta function twisted by a Dirichlet polynomial of length $\ll T^{1/2}$ so can be bounded in a similar way to \citep[proposition 2]{heap-soundararajan} using theorem 1 of \citep{twisted-second-moment}. This is carried out below. 
% Previous version %
%All that remains is to bound (\ref{eq:2}) and (\ref{eq:6}), which may be viewed as an easier version of proposition 3 of \cite{heap-radziwill-soundararajan}, or of proposition 3 of \cite{curran-1}.
% In fact all the key ingredients to bound  (\ref{eq:2}) and (\ref{eq:6}) are already present in \cite{curran-1}.

% Filled in the proposition and started the proof. The plan is to sketch Heap-Sound's strategy for eq:2 and then use that the range of primes in $\p_r$ is disjoint from the $\n_j$ so hopefully either essentially can be factored out at some point or becomes negligible.


% Here's an easier strategy: Use the formula from lemma one on my joint moments paper (the one for I_T(alpha beta), not I tilde) to bound the integral by log T times the max of F(z_1, z_2) with z_j \asymp 1/\log T. Then just use the bounds for F that are already in my earlier paper. 


\begin{prop} \label{prop:MVCalculations}
    For $1\leq r \leq J$,
    \begin{equation}
        %I_r:=
        \int_T^{2T} |\zeta(\tfrac{1}{2} + i t)|^2 \prod_{j < r} |\n_j(\tfrac{1}{2}+ i t;k - 1)|^2 \left|\frac{\p_r(s)}{50 P_r} \right|^{2\ceil{50P_r}} \ \dd t \ll e^{-10P_r}T(\log T)^{k^2}.
    \end{equation}
\end{prop}
\begin{proof}
If one takes $\phi(t)$ to be a smooth majorant of $1_{[1,2]}$ supported on $[1/2,3/2]$, the proof of Lemma 3.1 of \cite{curran-1} shows that for a Dirichlet polynomial $A(s)$ of length $\leq T^{1/2 - \ve}$,
\[
\int_{T}^{2T} |\zeta(\tfrac{1}{2} + i t)|^2 |A(\tfrac{1}{2} + i t)|^2 \ d t \ll T \log T \max_{|z_1|,|z_2| \asymp 1/\log T} |F(z_1,z_2)|.
\]
We wish to apply this to study the Dirichlet polynomial 
\[
\left(\prod_{j <  r} \n_j(\tfrac{1}{2}+ i t;k - 1) \right) \p_r(s) ^{\ceil{50P_r}}.
\]
Now we may simply note that in the proof of Proposition 2.4 of \cite{curran-1}, it is shown for this choice of Dirichlet polynomial that $|F(z_1,z_2)|$ is of order at most
\[
\prod_{j < r} \left(\prod_{T_{j-1} < p \leq T_j} \left(1+ \frac{k^2 - 1}{p} + O\left(\frac{1}{p^2}\right) \right) + O(e^{-100P_j}) \right) \times 2^{\ceil{50P_r}} \ceil{50P_r}! P_r^{\ceil{50P_r}} \exp(P_r)
\]
uniformly in $|z_j| \asymp 1/\log T$. 
The claim now follows from Merten's estimates and Stirling's approximation.
\end{proof}
\noindent
We now have all the necessary estimates to prove Theorem \ref{thm:mainUnconditional}.

\begin{proof}[Proof of Theorem \ref{thm:mainUnconditional}]  
Combining Proposition \ref{prop:MVCalculations} with the aforementioned bounds in \cite{curran-1, heap-radziwill-soundararajan, heap-soundararajan}, we see that the integral over the $\G$ satisfies
\begin{align*}
\int_\G |\zeta(\tfrac{1}{2} + i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \ll \left(T (\log T)^{k^2 + 2}\right)^h \left(T(\log T)^{k^2}\right)^{1-h} \ll T (\log T)^{k^2 + 2 h}.
\end{align*}
Similarly for each $1\leq r\leq J$, an application of Stirling's approximation gives
\begin{align*}
\int_{\B_r} |\zeta(\tfrac{1}{2} &+ i t)|^{2k - 2h} |\zeta'(\tfrac{1}{2} + i t)|^{2h} \ d t \\
&\ll \left(T (\log T)^{k^2 + 2} e^{-10P_r}\right)^h \left(T(\log T)^{k^2}  e^{-10P_r}\right)^{1-h} \ll T (\log T)^{k^2 + 2 h}  e^{-10P_r}.
\end{align*}
The claim now follows since $\G$ and $\B_r$ partition $[T,2T]$ while $\sum_{r\leq J}  e^{-10P_r} = O(1)$.
\end{proof}




==> very_old/2023-05-01_changes.tex <==
What I've changed (not much):

- files we weren't using in main are in the `old' folder
- where I've made a change, I've either left the old thing but commented it out, or left a comment detailing exactly what I changed.


==> very_old/introduction.tex <==
\section{Introduction}

\subsection{Background}
For $k\in \R_{\geq 0}$, the moments 
\begin{equation}
    M_k=M_k(T):=\int_{T}^{2T} |\zeta(1/2+it)|^{2k}\ d t
\end{equation}
have been well-studied, and conjectured to satisfy
\begin{equation}\label{zeta_moment_bound}
    M_k(T)\asymp_k T\log^{k^2}T.
\end{equation}
For $k\in\N$, there are conjectural values for the implied constant. Currently, the lower bound in \eqref{zeta_moment_bound} is known \citep{heap-soundararajan} unconditionally for all $k>0$. For $k\in[0,2]$, the upper bound is known unconditionally \citep{heap-radziwill-soundararajan}, with the upper bound for $k>2$ conditional on the Riemann Hypothesis \citep{harper}.

More recently, the joint moments
\begin{equation}
    M_{k,h}(T):= \int_{T}^{2T} |\zeta(1/2+it)|^{2k-2h}|\zeta'(1/2+it)|^{2h}\ d t
\end{equation}
have been studied.
In the range $k,h\geq -1/2$ with $h\leq k+1/2$, these are conjectured to satisfy
\begin{equation}
    M_{k,h}(T) \asymp_{k,h} T\log^{k^2+2h} T,
\end{equation}
with applications including the spacing between roots of $\zeta(s)$ on the critical line \citep{hall}. For integral $k$ and $h$ there are again conjectural values for the implied constant.

It should be noted that if $h\geq k$, then $M_{k,h}$ contains a small negative power of $\zeta(1/2+it)$. For the negative moments $M_{-k}(T)$, the best results to date, slightly shifted off the critical line and conditional on the Riemann Hypothesis, are those of Bui and Florea \citep{bui-florea}, which are still not conjecturally sharp. In particular, for $M_{k,h}(T)$, we speculate that the range $k\geq h \geq 0$ seems to be the largest possible range in which a sharp upper bound for $M_{k,h}(T)$ is attainable with current methods. %what about $k\geq 0, h\in(-1/2,0)$?

In the range $(k,h)\in [1,2]\times[0,1]$, Curran \citep{curran-1} has obtained an upper bound matching the conjecture, by using H\"older's inequality to compare
\begin{equation}\label{h_holder}
  M_{k,h}\ll (M_{k,1})^{h}(M_{k})^{1-h}
\end{equation}
and then using Young's inequality to upper bound $M_{k,1}$ by moments of short Dirichlet polynomials and a twist of $|\zeta(1/2+it)|^2|\zeta'(1/2+it)|^2$ by a short Dirichlet polynomial, which can then each be evaluated.


\subsection{Results}

The main result of this note is the theorem below. The valid ranges of $k$ and $h$ are divided up into parts, since in each part the method of proof differs. These parts are drawn on the subsequent figure, along with ranges of previously known results. %need to make this

\begin{thm}\label{thm_main}
    Let $k,h\in \R_{\geq 0}$, with $0 \leq h \leq k$. The upper bound
        \begin{equation}\label{main_UB}
            M_{k,h}(T)\ll_{k,h} T\log^{k^2+2h}T
        \end{equation}
    holds in the ranges:
    \begin{enumerate}
        \item $0 \leq k < 1/2$,
        \item $1/2 < k \leq 2$, and
        \item assuming the Riemann Hypothesis, $2 < k$.
    \end{enumerate}
\end{thm}


% For higher derivatives, we have the following result.

% \begin{thm}\label{higher_derivatives_main_thm}
%     Let $k>0$ and $h_1,\dots,h_n>0$ be such that $\sum_{j=1}^n h_j \leq k $. Let
%     \begin{equation}
%         M_{k,h_1,\dots,h_n}(T):= \int_{T}^{2T} |\zeta(1/2+it)|^{2k-\sum_{j=1}^N 2h_j}\prod_{j=1}^n |\zeta^{(j)}(1/2+it)|^{2h_j}.
%     \end{equation}
%     We have the upper bound
%     \begin{equation}
%         M_{k,h_1,\dots,h_n}(T)\ll_{k,h_1,\dots,h_n} T(\log T)^{\sum_{j=1}^n (j+1)h_j}
%     \end{equation}
%     in the ranges:
%     \begin{enumerate}
%         \item $0\leq k \leq 1/2$
%         \item $1/2 \leq k \leq 2$
%         \item assuming the Riemann hypothesis, $k\geq 2$.
%     \end{enumerate}
% \end{thm}



==> very_old/notes.tex <==
Remaining tasks:

- write out lemma 2
- finish justifying replacement of exps by N
- prove \eqref{2,0-moment} in the context of lemma 4
- prove \eqref{2,2-moment} and \eqref{0,2-moment} in lemmas 3 and 4

Extra ideas:

- how much effort does it take to get higher derivatives? ($k\geq 1/2$ is very easy; $k\leq 1/2$ is doable?











==> very_old/proof_big_k.tex <==
\section{Proof of Theorem 1 in ranges (ii) and (iii)}

First assume that $k\geq 1/2$, and that $h\in(0,1)$; if $h=0$, then $M_{k,h}=M_k$ has a known upper bound of the correct size \citep{heap-radziwill-soundararajan}.

In a very similar way to H\"older's inequality \eqref{h_holder} as in \citep{curran-1}, we have for any $\alpha\in(h,k)$,
\begin{equation}\label{change_h_holder}
    M_{k,h}(T)\leq (M_{k,\alpha}(T))^{h/\alpha}(M_k(T))^{1-h/\alpha}.
\end{equation}
The point of this is that, since $M_k(T)$ has a known  upper bound under RH \citep{harper}, to prove that $M_{k,h}(T)\ll T\log^{k^2+2h}(T)$ it now suffices to show that 
\begin{equation}
    M_{k,\alpha}(T)\ll_{k,\alpha} T\log^{k^2+2\alpha}(T), \quad M_{k}(T)\ll_k T\log^{k^2} T.
\end{equation}
The second bound is the main result of \citep{heap-radziwill-soundararajan}, and the first bound is the upper bound we intend to prove for $M_{k,\alpha}(T)$, provided that $\alpha>1/2$; it is possible to choose such an $\alpha$ since $k>1/2$. The proof is thus reduced to the case where $h > 1/2$.

Hence we can assume without loss of generality that $1/2\leq h \leq k$. Let $T>0$ be sufficiently large, $R=c/\log T$, for an arbitrarily chosen, fixed $c\in(0,1)$. The particular choice of $R$ cannot (up to the constant) be any smaller, else our argument will no longer be sharp, but cannot be larger else the shifted moments of the Riemann zeta function that we end up with might have the wrong sizes. Furthermore let $\gamma$ denote the anti-clockwise circular contour of radius $R$ centred at the origin.

Our starting point is the identity
\begin{equation}
    \zeta'(1/2+it) = \frac{1}{2\pi i}\oint_{\gamma} \frac{\zeta(1/2+it+z)}{z^2} \ d z.
\end{equation}
This implies that
\begin{align}
    |\zeta'(1/2+it)|^{2h} &= \frac{1}{(2\pi)^{2h}}\left|\oint_{\gamma}\frac{\zeta(1/2+it+z)}{z^2}\ d z\right|^{2h}\\
    &\leq \frac{R^{-4h}}{(2\pi)^{2h}}\left|\oint_{\gamma}|\zeta(1/2+it+z)|\ d |z|\right|^{2h}\\
    &\leq \frac{R^{-4h}}{(2\pi)^{2h}}\left|\oint_{\gamma}|\zeta(1/2+it+z)|^{2h}\ d |z|\right|\cdot \left|\oint_{\gamma} 1 \ d |z|\right|^{2h-1}\\
    &= \frac{R^{-2h-1}}{(2\pi)^{2h}}\oint_{\gamma}|\zeta(1/2+it+z)|^{2h}\ d |z|,
\end{align}
where the penultimate step is H\"older's inequality applied to $\zeta'(1/2+it+z)\times 1$ with exponents $p=2h$ and $q=2h/(2h-1)$. This is the only time we use the requirement that $h > 1/2$.

Using the above,
\begin{align}
    M_{k,h}(T) &= \int_{T}^{2T} |\zeta(1/2+it)|^{2k-2h}|\zeta'(1/2+it)|^{2h}\ d t\\
    &\leq \frac{R^{-2h-1}}{(2\pi)^{2h}}\int_{T}^{2T}|\zeta(1/2+it)|^{2k-2h}\oint_{\gamma }|\zeta(1/2+it+z)|^{2h}\ d |z| \ d t\\
%    &= \frac{R^{-2h-1}}{(2\pi)^{2h}}\int_{T}^{2T}\oint_{\gamma}|\zeta(1/2+it)|^{2k-2h}|\zeta(1/2+it)|^{2h}\ d |z| \ d t\\
    &= \frac{R^{-2h-1}}{(2\pi)^{2h}}\oint_{\gamma}\int_{T}^{2T}|\zeta(1/2+it)|^{2k-2h}|\zeta(1/2+it+z)|^{2h}\ d t \ d |z|\\
    &\leq \frac{R^{-2h}}{(2\pi)^{2h}}\max_{|z| = R}\int_{T}^{2T} |\zeta(1/2+it)|^{2k-2h}|\zeta(1/2+it+z)|^{2h}\ d t.
\end{align}

Hence $M_{k,h}(T)$ has been expressed in terms of shifted moments of $\zeta(1/2+it+z)$, with small shifts $z$. If $h=k$, then the theorem follows from applying either the bounds for $M_k$ from  \citep{heap-radziwill-soundararajan} or \citep{harper} depending on whether we are in range (ii) or (iii) respectively.
%% I Don't think this last assertion is justified – you can fix it conditionally by using my last paper on shifted moments. Undconditionally I think we have to work a bit harder here, though it's probably possible to prove an unconditional estimate for shifted moments with two shifts and different exponents with not too much work.
If $h < k$, then by H\"older's inequality with exponents $p=k/(k-h)$ and $q=k/h$, we now have
\begin{equation}
    \begin{split}
        \int_{T}^{2T} |\zeta(1/2+it)&|^{2k-2h}\cdot |\zeta(1/2+it)|^{2h}\ d t \\
        &\leq \left(\int_T^{2T}|\zeta(1/2+it)|^{2k}\ d t\right)^{(k-h)/k}\left(\int_{T}^{2T}|\zeta(1/2+it+z)|^{2k}\ d t\right)^{k/h}\\
        &\ll T\log^{k^2} T,
    \end{split}
\end{equation}
where the last line is again either by \citep{heap-radziwill-soundararajan} in range (ii), or \citep{harper} in range (iii).
Note that since $\zeta(1/2+it)$ and $\zeta(1/2+it+z)$ are expected to have correlated powers for small shifts, H\"older's inequality ends up being sharp.

%%% %%% %%% %%% 
\raggedleft
 $\square$

 
\raggedright
%%% %%% %%% %%%


==> very_old/proof_higher_derivatives.tex <==
We now describe how to modify the approaches of the previous sections to obtain theorem \ref{higher_derivatives_main_thm}.

In ranges (ii) and (iii), we instead start with
\begin{equation}
    \zeta^{(n)}(s)= \frac{1}{2\pi i}\oint_{\gamma_R} \frac{\zeta(s+z)}{z^n}\d z...
\end{equation}

==> very_old/proof_small_k.tex <==
\section{Proof of Theorem 1 in range (i)}

\subsection{Notation}
The immediate problem in generalising the strategy of the previous subsection to $k\leq 1/2$ is that it is no longer possible to choose an $\alpha\in(h,k)$ such that \eqref{change_h_holder} works. In order to work around this, we first apply Young's inequality, which essentially has the effect of increasing $k$ so that we can then apply H\"older's inequality to the individual resulting terms and evaluate the resulting moments.

We first recall the standard notation from \citep{heap-soundararajan} and introduce a little more. Let $T_j:= \exp(\log T / \log_j T)$ for $2\leq j \leq \ell$, where $\ell$ is the largest integer such that $T_j\ll T^{10^{-8}}$; for each such $j$ define
\begin{equation}
    P_j(s):= \sum_{p \in (T^{j-1},T^j]} p^{-s}.
\end{equation}
Further, let $P_j:=P_j(1)$ for $2\leq j \leq \ell$, and let 
\begin{equation}
    N_j(s;\alpha):= E_{\ell_j}(\alpha P_j(s)),
\end{equation}
where $E_{\ell_j}$ is the degree $\ell_j$ Taylor polynomial of $\exp$. Finally, let
\begin{equation}
    N(s;\alpha):= \prod_{j=2}^\ell N_j(s;\alpha), \quad P(s):= \sum_{j=2}^\ell P_j(s)
\end{equation}
and for $2\leq j < \ell$ let
\begin{equation}
    \tN_{j}(s;\alpha):= \prod_{v=2}^j N_v(s;\alpha), \quad \tP_j(s):= \sum_{v=2}^j P_j(s),
\end{equation}
so that $\tN_j$ is an approximation to $\exp(\alpha\tP_j)$.

\subsection{Reduction to twisted moments}
The precise form of Young's inequality that we will use is essentially that of \citep[Lemma 2]{radziwill-soundararajan}, and is as follows.
\begin{lem}\label{lem_change_k}
    Let. $0\leq h \leq k \leq 1/2$.
    For all $s$ inside the critical strip, 
    \begin{equation}\label{change_k}
        \begin{split}
        |\zeta(s)|^{2k-2h} \ll_{k,h} & |\zeta(s)|^2\exp(2(k-h-1)P(s)) +  \exp(2(k-h)P(s))\\
        &+ \sum_{j=2}^{\ell-1} \left(|\zeta(s)|^2\exp(2(k-h-1)\tP_j(s)) + \exp(2(k-h)\tP_j(s))\right) \left|\frac{P_j(s)}{50P_j}\right|^{2\lceil 50 P_j \rceil}.
        \end{split}
    \end{equation}
\end{lem}
\begin{proof}
    ...
\end{proof}
In fact, by examining the proof, the lemma remains true provided that $k-h\leq 1$.

To obtain a sharp upper bound for $M_{k,h}(T)$, it now suffices to find sharp upper bounds for each term on the right hand side of \ref{change_k} after multiplying through by $|\zeta'(s)|$ and integrating from $1/2+iT$ to $1/2+2iT$. As stated, these involve fractional powers of $\zeta'$, but these can be removed by additional applications of H\"older's inequality.

Applying H\"older's inequality to the first term we have
\begin{equation}
    \begin{split}
        \int_T^{2T}|\zeta(1/2+it)|^2&|\zeta'(1/2+it)|^{2h}\exp(2(k-h-1)P(1/2+it))\d t \leq \\
    \ll &\left(\int_T^{2T} |\zeta(1/2+it)|^2|\zeta'(1/2+it)|^2\exp(2(k-2)P(1/2+it))\d t\right)^{h}\\
        &\times\left(\int_T^{2T} |\zeta(1/2+it)|^2\exp(2(k-1)P(1/2+it))\d t\right)^{1-h},
    \end{split}
\end{equation}
and to the second term,
\begin{equation}
    \begin{split}
        \int_T^{2T} |\zeta'(1/2+it)|^{2h}&\exp(2(k-h-1)P(1/2+it))\d t \\
        \ll&\left(\int_T^{2T} |\zeta'(1/2+it)|^2\exp(2(k-2)P(1/2+it))\d t\right)^{h}\\
        &\left(\int_T^{2T} \exp(2kP(1/2+it))\d t\right)^{1-h}.
    \end{split}
\end{equation}
Similar identities hold for the third and fourth terms, with $P$ replaced by $\tP$ and with an extra factor of $|P_j(s)/(50P_j)|^{2\lceil 50 P_j \rceil}$ in each integrand on the right hand side.

We can now replace the exponentials by truncated Taylor series involving the $N_j$. To be precise, we split $P(s)$ and the $\tP_j(s)$ up into the $P_j$, and separately approximate each term of the form $\exp(2\alpha P_j(s))$ by $|N_j(s;\alpha)|^2$. Each of these introduces an error of size
\begin{equation}
    ...
\end{equation}
and summing these over $2\leq j \leq \ell$ is bounded above by an absolute constant.

As a result, this replacement does not affect the asymptotic size of each term, and theorem \ref{thm_main} follows from the next lemma.
\begin{lem}\label{lem_moments_UBs}
    For $k\in(0,1/2)$, $2\leq j\leq \ell-1$, we have the following upper bounds.
    \begin{align}\label{2,2-moment}
            \int_{T}^{2T} |\zeta(1/2+it)|^2|\zeta'(1/2+it)|^2|N(1/2+it;k-2)|^2\d t &\ll_{k} T\log^{k^2+2}T,\\ 
        \label{0,2-moment}
            \int_{T}^{2T} |\zeta'(1/2+it)|^2|N(1/2+it,k-1)|^2\d t &\ll_{k} T\log^{k^2+2} T,\\
        \label{2,0-moment}
            \int_{T}^{2T} |\zeta(1/2+it)|^2|N(1/2+it,k-1)|^2\d t &\ll T\log^{k} T\\
        \label{0,0-moment}
            \int_{T}^{2T} |N(1/2+it,k)|^{2}\d t &\ll_k T\log^{k^2} T.
    \end{align}
\end{lem}
\begin{lem}
    These all remain true upon replacing each term of the form $|N(1/2+it,\alpha)|^2$ by
    \begin{equation}
        |\tN_j(1/2+it,\alpha)|^2\left|\frac{P_j(s)}{50P_j} \right|^{2\lceil 50 P_j \rceil},
    \end{equation}
    and the upper bound is then of the form
    \begin{equation}
        \ll
    \end{equation}
\end{lem}
These upper bounds are proved in the next subsection; again by examining the proofs they are valid in a wider range of $k$ and $h$ than we require to prove \ref{thm_main}.

\subsection{Upper bounds for twisted moments}

In lemma \ref{lem_moments_UBs}, \eqref{0,0-moment} is a moment of a short Dirichlet polynomial, which can be evaluated easily, and \eqref{2,0-moment} is a twisted second moment. These moments are evaluated in \citep[Proposition 2]{heap-radziwill-soundararajan} and \citep[Proposition 2]{heap-soundararajan} respectively.

Equations \eqref{2,0-moment} and \eqref{2,2-moment} are evaluated using \citep[Lemma 1]{curran-1} and \citep[Lemma 2]{curran-2}, respectively.

